What Are People Asking About COVID-19? A Question Classification Dataset

We present COVID-Q, a set of 1,690 questions about COVID-19 from 13 sources, which we annotate into 15 question categories and 207 question clusters. The most common questions in our dataset asked about transmission, prevention, and societal effects of COVID, and we found that many questions that appeared in multiple sources were not answered by any FAQ websites of reputable organizations such as the CDC and FDA. We post our dataset publicly at https://github.com/JerryWeiAI/COVID-Q. For classifying questions into 15 categories, a BERT baseline scored 58.1% accuracy when trained on 20 examples per category, and for a question clustering task, a BERT + triplet loss baseline achieved 49.5% accuracy. We hope COVID-Q can help either for direct use in developing applied systems or as a domain-specific resource for model evaluation.

==> figures/BERT_example_predictions.tex <==
%Examples for BERT correct and incorrect predictions: columns should be question, ground-truth class, predicted class, predicted closest questions
\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{2pt}
    % \scriptsize
    \footnotesize
    \begin{tabular}{l | c c | c}
         \toprule
         Question & Ground-Truth Class & Predicted Classes & Predicted Closest Questions\\
         \midrule
         \multirow{3}{*}{``Is COVID curable?"} & \multirow{3}{*}{Existence of Treatments} & Number of Cases & ``Are COVID numbers going down?"\\
         & & Worse than Flu & ``Is COVID worse than flu?"\\
         & & Availability of Tests & ``Is there a test for COVID?"\\ 
         \midrule
         \multirow{3}{*}{``Can I still travel?"} & \multirow{3}{*}{Cancelling Trips} & General Prevention & ``How do I stop COVID?"\\
         & & Pandemic Duration & ``Will COVID end soon?"\\
         & & Survivability: Temperature & ``Can COVID survive cold?"\\
         \midrule
         \multirow{3}{*}{\begin{minipage}{1.3in}``What is the start\\ date of COVID?"\end{minipage}} & \multirow{3}{*}{Origin - Time} & Pandemic Duration & ``What is the official end date to COVID?"\\
         & & Reason for Name & ``What is the acronym COVID?"\\
         & & General Symptoms & ``What are the symptoms of COVID?"\\ 
         \bottomrule
    \end{tabular}
    \caption{Incorrect predictions from baseline BERT model.}
    \label{tab:BERT_predictions}
\end{table*}
